Semi-Supervised Learning with Deep Generative Models

The ever-increasing size of modern data sets combined with the difficulty of obtaining label information has made semi-supervised learning one of the problems of significant practical importance in modern data analysis. We revisit the approach to semi-supervised learning with generative models and develop new models that allow for effective generalisation from small labelled data sets to large unlabelled ones. Generative approaches have thus far been either inflexible, inefficient or non-scalable. We show that deep generative models and approximate Bayesian inference exploiting recent advances in variational methods can be used to provide significant improvements, making generative approaches highly competitive for semi-supervised learning.

==> nips2014-semisupervised copy/discussion.tex <==
\section{Discussion and Conclusion}
\label{sect:discussion}
\vspace{-2mm}
%
The approximate inference methods introduced here can be easily extended to the model's parameters, harnessing the full power of variational learning. Such an extension also provides a principled ground for performing model selection. Efficient model selection is particularly important when the amount of available data is not large, such as in semi-supervised learning. 

For image classification tasks, one area of interest is to combine such methods with convolutional neural networks that form the gold-standard for current supervised classification methods. Since all the components of our model are parametrised by neural networks we can readily exploit convolutional or more general locally-connected architectures -- and forms a promising avenue for future exploration.
%This is possible by representing the approximate posterior distributions using convolutional models, and any independent discriminative components can also be represented as convolutional models.

A limitation of the models we have presented is that they scale linearly in the number of classes in the data sets. Having to re-evaluate the generative likelihood for each class during training is an expensive operation. Potential reduction of the number of evaluations could be achieved by using a truncation of the posterior mass. For instance we could combine our method with the truncation algorithm suggested by \cite{pal2005fast}, or by using mechanisms such as error-correcting output codes \citep{dietterich1995solving}. The extension of our model to multi-label classification problems that is essential for image-tagging is also possible, but requires similar approximations to reduce the number of likelihood-evaluations per class.
%In order to achieve the property that the classification component learns at all times, we have introduced the augmented loss \eqref{eq:simplifyiedBoundGenerativeAugmented}. It would  be  desirable to have a single principled loss function similar to  \citep{blum2004semi} or \citep{zhu2003semi}.

We have developed new models for semi-supervised learning that allow us to improve the quality of prediction by exploiting information in the data density using generative models. We have developed an efficient variational optimisation algorithm for approximate Bayesian inference in these models and demonstrated that they are amongst the most competitive models currently available for semi-supervised learning. We hope that these results stimulate the development of even more powerful semi-supervised classification methods based on generative models, of which there remains much scope.

\paragraph{Acknowledgements.} We are grateful for feedback from
the reviewers. We would also like to thank the SURFFoundation for the use of the Dutch national e-infrastructure for a significant part of the experiments.

==> nips2014-semisupervised copy/inference.tex <==
\vspace{-2mm}
\section{Scalable Variational Inference}
\label{sect:inference}
\vspace{-2mm}

\subsection{Lower Bound Objective}
\vspace{-2mm}
In all our models, computation of the exact posterior distribution is intractable due to the nonlinear, non-conjugate dependencies between the random variables. To allow for tractable and scalable inference and parameter learning, we exploit recent advances in variational inference \citep{kingma2014, rezende2014}.
For all the models described, we introduce a fixed-form distribution $q_{\phi} (\vz | \vx)$ with parameters $\vphi$ that approximates the true posterior distribution $p(\vz | \vx)$. We then follow the variational principle to derive a lower bound on the marginal likelihood of the model -- this bound forms our objective function and ensures that our approximate posterior is as close as possible to the true posterior. 

We construct the approximate posterior distribution $q_{\phi}(\cdot)$ as an inference or recognition model, which has become a popular approach for efficient variational inference \citep{kingma2014, rezende2014, Dayan2000, stuhlmuller2013learning}. Using an inference network, we avoid the need to compute per data point variational parameters, but can instead compute a set of global variational parameters $\vphi$. This allows us to amortise the cost of inference by generalising between the posterior estimates for all latent variables through the parameters of the inference network, and  allows for fast inference at both training and testing time (unlike with VEM, in which we repeat the generalized E-step optimisation for every test data point).
%Given the specification of the models in the previous section, we can perform inference and parameter learning using the marginal likelihood as the objective function, which involves an integration over the latent variables. To allow for tractability, we follow the variational principle of introducing an approximate posterior distribution $q_{\small \vphi} (\vz | \vx)$ with variational parameters $\vphi$ and obtain a lower bound on the marginal likelihood, which we use as the objective function. 
%The variational distribution $q_{\vphi} (\vz  | \vx)$ is conditioned on the observed data and shares statistical strength across the posterior estimates for all latent variables through its parameters. It also allows for fast inference during both training and test time (unlike with VEM, in which we repeat the generalized E-step optimisation for every test data point).
An inference network is introduced for all latent variables, and we parameterise them as deep neural networks whose outputs form the parameters of the distribution $q_{\phi}(\cdot)$.
For the latent-feature discriminative model (M1), we use a Gaussian inference network $q_{\phi} (\vz  | \vx)$ for the latent variable $\vz$. For the generative semi-supervised model (M2), we introduce an inference model for each of the latent variables $\vz$ and $y$, which we we assume has a factorised form $q_{\phi} (\vz, y | \vx) = q_{\phi} (\vz  | \vx)q_{\phi} (y | \vx)$, specified as Gaussian and multinomial distributions respectively.
\begin{align}
\textrm{M1: } & q_{\phi} (\vz  | \vx) = \N(\vz | \vmu_{\phi}(\vx), \diag(\vsigma_{\phi}^2(\vx)) ), \label{eq:recogModel1} \\
\textrm{M2: } & q_{\phi} (\vz  | y, \vx) = \N(\vz | \vmu_{\phi}(y, \vx), \diag(\vsigma_{\phi}^2(\vx))); \,\,\, q_{\phi} (y | \vx) = \textrm{Cat}(y | \vpi_{\phi}(\vx)),  \label{eq:recogModel2}
\end{align}
where $\vsigma_{\phi}(\vx)$ is a vector of standard deviations, $\vpi_{\phi}(\vx)$ is a probability vector, and the functions $\vmu_{\phi}(\vx)$, $\vsigma_{\phi}(\vx)$ and $\vpi_{\phi}(\vx)$ are represented as MLPs.
%
%For the conditional generative model (M2), we define an inference network $q_{\phi} (\vz  | y, \vx)$ for the Gaussian latent variables $\vz$ that is also conditioned on the label $y$ and a second inference network $q_{\phi} (y | \vx)$ for the missing labels
%\begin{align}
%q_{\small \phi} (\vz  | y, \vx) = \N(\vz | \vmu_{\vphi}(y, \vx), \diag(\vsigma_{\vphi}(\vx)^2)); \qquad q_{\small \phi} (y | \vx)) = \textrm{Cat}(y | \vpi_{\vphi}(\vx)),  \label{eq:recogModel}
%\end{align}
%where $\vpi_{\vphi}(\vx)$ is a probability vector parametrized by a MLP.
%We parameterise the inference networks using fully connected neural networks with softplus non-linearities $g(\cdot)$. Hence, the inference network for $q_{\phi}(y | \vx)$ consists of a neural network that takes the observation $\vx$ as the input and produces the parameters $\vpi(\vx)$ of a discrete distribution over the $L$ classes. Similarly, the inference network for the latent variables $q_{\phi}(\vz | y, \vx)$ is a neural network that takes $y$ and $\vx$ as input and provides as output the canonical parameters $\vmu(\vx), \vR(\vx)$ of a Gaussian distribution. When using neural networks in the generative and recognition models, the resulting architecture is also referred to as a \emph{variational auto-encoder} (VAE).
\subsubsection{Latent Feature Discriminative Model Objective}
For this model, the variational bound $\mathcal{J}(\vx)$ on the marginal likelihood for a single data point is:
%For the latent feature discriminative model (M1), we only require an approximate posterior $q_{\small \phi} (\vz | \vx)$. The variational bound of the marginal likelihood of datapoint $\bx$ is obtained as:
\begin{align}
\log \pT(\bx) &\geq \expect{\qphi (\bz|\bx) }{ \log \pT(\bx|\bz)} - KL[\qphi(\bz|\bx) \| \pT(\bz) ]
= - \mathcal{J}(\bx), \label{eq:negFreeEnergy}
\end{align}
The inference network $\qphi(\vz|\vx)$ \eqref{eq:recogModel1} is used during training of the model using both the labelled and unlabelled data sets. This approximate posterior is then used as a feature extractor for the labelled data set, and the features used for training the classifier.
%and $q_{\small \phi} (\vz|\vx)$ is the variational approximate posterior (also referred to as the recognition/inference model/network). We use this objective for optimisation and use draws from $q_{\small \phi} (\vzi|\vxi)$ as features for the observed data, which we then use to train a classifier.
%It can be enlightning to realize that this objective can also be written as $- D_{KL}(\pdata(\bx)\qphi(\bz|\bx) || \pT(\bx,\bz)) + \mathcal{H}(\pdata)$; since the parameters do not affect $\mathcal{H}(\pdata)$ this term can be ignored, and optimization of the objective in~\eqref{eq:negFreeEnergy} is equivalent to minimization of the KL-divergence of the joint distribution $\pdata(\bx) \qphi(\bz|\bx)$ from the generative model distribution $\pT(\bx,\bz)$.
%It is straightforward to show that the bound is saturated iff $q_{\small \phi} (\vz|\vx) \propto p_{\theta}(\vz|\vx) $. Typically the distribution $q_{\small \phi} (\vz|\vx)$ is chosen such that the expectations in \ref{eq:negFreeEnergy} can be solved analytically or efficiently approximated.

\subsubsection{Generative Semi-supervised Model Objective}
For this model, we have two cases to consider. In the first case, the label corresponding to a data point is observed
and the variational bound is a simple extension of equation \eqref{eq:negFreeEnergy}:
\begin{align}
\log \pT(\bx,y) \!\geq\!\expect{\qphi(\bz|\bx,y)}{\log \pT(\bx|y,\bz) + \log \pT(y) + \log p(\bz) - \log \qphi(\bz|\bx,y) } \!=\!-\Fl(\bx,y),
\end{align}
%where the generative model is factorized as $\log \pT(\bx,y,\bz) = \log \pT(\bx|y,\bz) + \log \pT(y) + \log p(\bz)$. We also refer to the bound $\Fl(\bx,y)$ as the conditional bound.
%In our experiments, $\qphi (\vz|y,\vx)$ is parameterised with a deep neural network.
%When the label $y$ is latent, like $\vz$, a joint posterior over $y$ and $\vz$ must be inferred.
%For this we introduce the variational distribution $\qphi (y,\vz|\vx)$, which we factorize as $\qphi(y,\vz|\vx) = \qphi(y| \vx) \qphi (\vz|y,\vx)$. We also parameterise the distribution $\qphi (y|\vx)$ with a deep neural network in our experiments. 

For the case where the label is missing, it is treated as a latent variable over which we perform posterior inference and the 
resulting bound for handling data points with an unobserved label $y$ is:
\begin{align}
\log \pT(\vx)
&\geq \expect{\qphi(y,\bz|\bx)}{\log \pT(\bx|y,\bz) + \log \pT(y) + \log p(\bz) - \log \qphi(y,\bz|\bx)} \nonumber \\
&= \sideset{}{_y}\sum \qphi(y|\bx) ( -\Fl(\bx,y)) + \mathcal{H}(\qphi(y|\bx)) = - \Fu(\bx).
\end{align}
The bound on the marginal likelihood for the entire dataset is now:
\begin{align}
% N_{labeled} \cdot \expect{\pldata(\bx,y)}{ - \Fl(\bx,y) }
%+ N_{unlabeled} \cdot \expect{\pudata(\bx)}{ - \Fu(\bx) }
\mathcal{J} =
\sideset{}{_{(\bx,y) \sim \pldata}}\sum \Fl(\bx,y)
+ \sideset{}{_{\bx \sim \pudata}}\sum \Fu(\bx)
\label{eq:simplifiedBoundGenerative}
\end{align}

The distribution $\qphi(y|\bx)$ \eqref{eq:recogModel2} for the missing labels has the form a discriminative classifier, and we can use this knowledge to construct the best classifier possible as our inference model. This distribution is also used at test time for predictions of any unseen data.
%\begin{align}
%& \log \pT(\vx) \geq 
% \sum_{n \in \mathcal{O}}  \mathcal{F}(\vxi, \yi)
%+ \sum_{n \notin \mathcal{O}} \expect{\qphi (y|\vxi)}{
%\mathcal{F}(\vxi, y) + \log \qphi (y |\vxi) } = 
%\mathcal{F}
%\label{eq:simplifyiedBoundGenerative}
%\end{align}

In the objective function \eqref{eq:simplifiedBoundGenerative}, the label predictive distribution $q_{\small \phi} (y|\vx)$ contributes only to the second term relating to the unlabelled data, which is an undesirable property if we wish to use this distribution as a classifier. Ideally, all model and variational parameters should learn in all cases. To remedy this, we add a classification loss to \eqref{eq:simplifiedBoundGenerative}, such that the distribution $q_{\small \phi} (y|\vx)$ also learns from labelled data. The extended objective function is:
\begin{align}
\mathcal{J}^\alpha
&= \mathcal{J} + \alpha \cdot \expect{\pldata(\bx,y)}{ - \log \qphi(y|\bx) },
\label{eq:simplifyiedBoundGenerativeAugmented}
\end{align}
%\begin{align}
%\textrm{\textbf{M2}: } \mathcal{F}^{\alpha}  = (1-\alpha) \mathcal{F} - \alpha %\sum_{n \in \mathcal{O}} \log \qphi (\yi | \vxi)
%\label{eq:simplifyiedBoundGenerativeAugmented}
%\end{align}
where the hyper-parameter $\alpha$ controls the relative weight between generative and purely discriminative learning. We use $\alpha=0.1\cdot N$ in all experiments. While we have obtained this objective function by motivating the need for all model components to learn at all times, the objective \ref{eq:simplifyiedBoundGenerativeAugmented} can also be derived directly using the variational principle by instead performing inference over the parameters $\vpi$ of the categorical distribution, using a symmetric Dirichlet prior over these parameterss.
%\hl{Note: The alternative approach where the prior of $y$ %is seen as an always-latent variable could be added here, %similar to the proposal by Phil Bachman. A problem is %that it comes with a slightly altered objective (the weight %of $\Fl(\bx,y)$ is increased), and all experiments would %need to be re-run (although with probably similar %results). So probably better to keep the objective as is, %and maybe change the arXiv version later if we want?}
\subsection{Optimisation}
%\subsection{Free Energy Optimisation}
\label{sect:infer_optim}
The bounds in equations \eqref{eq:negFreeEnergy} and \eqref{eq:simplifyiedBoundGenerativeAugmented} provide a unified objective function for optimisation of both the parameters $\vtheta$ and $\vphi$ of the generative and inference models, respectively. This optimisation can be done jointly, without resort to the variational EM algorithm, by using deterministic reparameterisations of the expectations in the objective function, combined with Monte Carlo approximation -- referred to in previous work as \emph{stochastic gradient variational Bayes} (SGVB) \citep{kingma2014} or as \emph{stochastic backpropagation} \citep{rezende2014}.  We describe the core strategy for the latent-feature discriminative model M1, since the same computations are used for the generative semi-supervised model. 

When the prior $p(\vz)$ is a spherical Gaussian distribution $p(\vz) = \mathcal{N}(\vz| \vzero, \vI)$ and the variational distribution $q_{\phi} (\vz|\vx)$ is also a Gaussian distribution as in \eqref{eq:recogModel1}, the KL term in equation \eqref{eq:negFreeEnergy} can be computed analytically and the log-likelihood term can be rewritten, using the location-scale transformation for the Gaussian distribution, as:
\begin{align}
 \expect{q_{\phi} (\bz|\bx) } { \log p_{\theta}(\vx | \vz) }  &=  \expect{ \mathcal{N}( \vepsilon | \vzero, \vI ) } { \log p_{\theta}(\vx |  \vmu_{\phi}(\vx) + \vsigma_{\phi}(\vx) \odot \vepsilon ) }, \label{eq:reparametrization}
\end{align}
where $\odot$ indicates the element-wise product.
While the expectation \eqref{eq:reparametrization} still cannot be solved analytically, its gradients with respect to the generative parameters  $\vtheta$ and  variational parameters $\vphi$ can be efficiently computed as expectations of simple gradients:
\begin{align}
\nabla_{ \{\theta, \phi\} } \expect{q_{\small \phi} (\bz|\bx)}{\log p_{\theta}(\vx | \vz) }
 &=  \expect{ \mathcal{N}( \vepsilon | \vzero, \vI )  } { \nabla_{ \{\theta, \phi\} } \log p_{\theta}(\vx |  \vmu_{\phi}(\vx) + \vsigma_{\phi}(\vx) \odot \vepsilon)   }. \label{eq:reparametrizationGradThetaPhi}
\end{align}

The gradients of the loss \eqref{eq:simplifyiedBoundGenerativeAugmented} for model M2  can be computed by a direct application of the chain rule and by noting that the conditional bound $\Fl(\bx_n, y)$ contains the same type of terms as the loss \eqref{eq:simplifyiedBoundGenerativeAugmented}. The gradients of the latter can then be efficiently estimated using \eqref{eq:reparametrizationGradThetaPhi} . 

During optimization we use the estimated gradients in conjunction with standard stochastic gradient-based optimization methods such as SGD, RMSprop or AdaGrad~\citep{duchi2010adaptive}.
This results in parameter updates of the form: $
(\vtheta^{t+1}, \vphi^{t+1}) \gets (\vtheta^{t}, \vphi^{t}) + \boldsymbol{\Gamma}^t (\vg^t_{\theta}, \vg^t_{\phi} ), \nonumber
$
where $\vGamma$ is a diagonal preconditioning matrix that adaptively scales the gradients for faster minimization. The training procedure for models M1 and M2 are summarised in algorithms \ref{alg:train1} and \ref{alg:train2}, respectively. Our experimental results were obtained using AdaGrad.


\subsection{Computational Complexity}
\vspace{-2mm}
The overall algorithmic complexity of a single joint update of the parameters $(\vtheta, \vphi)$ for M1 using the estimator \eqref{eq:reparametrizationGradThetaPhi} is $C_{\textbf{M1}} = M S C_{\text{MLP}}$ where $M$ is the minibatch size used , $S$ is the number of samples of the random variate $\vepsilon$, and $C_{\text{MLP}}$ is the cost of an evaluation of the MLPs in the conditional distributions $p_{\theta}(\vx| \vz)$ and $q_{\small \phi} (\vz | \vx)$. The cost $C_{\text{MLP}}$ is of the form $O(KD^2)$ where $K$ is the total number of layers and $D$ is the average dimension of the layers of the MLPs in the model.
Training M1 also requires training a supervised classifier, whose algorithmic complexity, if it is a neural net, it will have a complexity of the form $C_{\text{MLP}}$ . 

The algorithmic complexity for M2 is of the form $C_{\text{M2}} = L C_{\text{M1}}$, where $L$ is the number of labels and $C_{\text{M1}}$ is the cost of evaluating the gradients of each conditional bound $\mathcal{J}_y(x)$, which is the same as for M1. The stacked generative semi-supervised model has an algorithmic complexity of the form  $C_{\textbf{M1}} + C_{\textbf{M2}}$. But with the advantage that the cost $C_{\textbf{M2}}$ is calculated in a low-dimensional space (formed by the latent variables of the model M1 that provides the embeddings). 

These complexities make this approach extremely appealing, since they are no more expensive than alternative approaches based on auto-encoder or neural models, which have the lowest computational complexity amongst existing competitive approaches. In addition, our models are fully probabilistic, allowing for a wide range of inferential queries, which is not possible with many alternative approaches for semi-supervised learning.



\begin{figure}[t]
\centering
\begin{minipage}{.47\textwidth}
  \centering
  \begin{algorithm}[H]
    \caption{Learning in model M1\!}
    \label{alg:train1}
  \begin{algorithmic}
  \WHILE{ generativeTraining() }
  \STATE $\D \gets \text{getRandomMiniBatch}()$
  \STATE $\vz_i \sim \qphi (\vz_i | \vx_i) \quad \forall \vx_i \in \D$
  \STATE $\mathcal{J} \gets \sum_n \mathcal{J}(\vx_i)  $
  \STATE $ (\vg_{\theta}, \vg_{\phi} ) \gets ( \frac{\partial \mathcal{J}}{\partial \theta},  \frac{\partial \mathcal{J}}{\partial \phi} )$
  \STATE $(\vtheta, \vphi) \gets (\vtheta, \vphi) + \vGamma (\vg_{\theta}, \vg_{\phi} )$
  \ENDWHILE
  
  \WHILE{ discriminativeTraining() }
  \STATE $\D \gets \text{getLabeledRandomMiniBatch}()$
  \STATE $\vz_i \sim q_{\small \phi} (\vz_i | \vx_i) \quad \forall  \{ \vx_i , y_i \} \in \D$
  \STATE $\text{trainClassifier}( \{ \vz_i, y_i \} $ )
  \ENDWHILE
  
  \end{algorithmic}
  \end{algorithm}
\end{minipage}%
\hskip5ex
\begin{minipage}{.47\textwidth}
 \begin{algorithm}[H]
   \caption{Learning in model M2 \!}
   \label{alg:train2}
 \begin{algorithmic}
 \WHILE{ training() }
 \STATE $\D  \gets \text{getRandomMiniBatch}()$
 \STATE $y_i~\sim~\qphi (y_i | \vx_i) \quad \forall \{ \vx_i , y_i \} \notin \mathcal{O}$
 \STATE $\vz_i \sim \qphi (\vz_i | y_i, \vx_i) $
 \STATE $\mathcal{J}^{\alpha}\gets $ eq. \eqref{eq:simplifyiedBoundGenerativeAugmented}
 \STATE $ (\vg_{\theta}, \vg_{\phi} ) \gets ( \frac{\partial \mathcal{L}^{\alpha}}{\partial \theta},  \frac{\partial \mathcal{L}^{\alpha}}{\partial \phi} )$
 \STATE $(\vtheta, \vphi) \gets (\vtheta, \vphi) + \vGamma (\vg_{\theta}, \vg_{\phi} )$
 \ENDWHILE
 \end{algorithmic}
 \end{algorithm}
\end{minipage}
\vspace{-5mm}
\end{figure}




==> nips2014-semisupervised copy/introduction.tex <==
\section{Introduction}
\label{sect:intro}
\vspace{-2mm}
\blfootnote{For an updated version of this paper, please see \url{http://arxiv.org/abs/1406.5298}}
Semi-supervised learning considers the problem of classification when only a small subset of the observations have corresponding class labels. Such problems are of immense practical interest in a wide range of applications, including image search \citep{fergus2009semi},  genomics \citep{ShiCancerSSL}, natural language parsing \citep{liang2005semi}, and speech analysis \citep{liu2013graph}, where unlabelled data is abundant, but obtaining class labels is expensive or impossible to obtain for the entire data set. The question that is then asked is: how can properties of the data be used to improve decision boundaries and to allow for classification that is more accurate than that based on classifiers constructed using the labelled data alone.
In this paper we answer this question by developing \textit{probabilistic models for inductive and transductive semi-supervised learning} by utilising an explicit model of the data density, building upon recent advances in deep generative models and scalable variational inference \citep{kingma2014, rezende2014}.
%by integrating out the assignment of any missing labels, use this generative model to improve the classification task.
%\comment{We don't have transductive experiments, but it could certainly be applied to transductive SSL, so we're indeed not being incorrect here} 

Amongst existing approaches, the simplest algorithm for semi-supervised learning is based on a \textit{self-training} scheme \citep{rosenberg2005semi} where the the model is bootstrapped with additional labelled data obtained from its own highly confident predictions; this process being repeated until some termination condition is reached. These methods are heuristic and prone to error since they can reinforce poor predictions. \textit{Transductive SVMs} (TSVM) \citep{joachims1999transductive} extend SVMs with the aim of max-margin classification while ensuring that there are as few unlabelled observations near the margin as possible. These approaches have difficulty extending to large amounts of unlabelled data, and efficient optimisation in this setting is still an open problem.  \textit{Graph-based methods} are amongst the most popular and aim to construct a graph connecting similar observations;  label information propagates through the graph from labelled to unlabelled nodes by finding the minimum energy (MAP) configuration \citep{blum2004semi, zhu2003semi}. Graph-based approaches are sensitive to the graph structure and require eigen-analysis of the graph Laplacian, which limits the scale to which these methods can be applied -- though efficient spectral methods are now available \citep{fergus2009semi}. \textit{Neural network}-based approaches combine unsupervised and supervised learning by training feed-forward classifiers with an additional penalty from an auto-encoder or other unsupervised embedding of the data \citep{ranzato2008semi, weston2012deep}. The Manifold Tangent Classifier (MTC)~\citep{rifai2011manifold} trains contrastive auto-encoders (CAEs) to learn the manifold on which the data lies, followed by an instance of TangentProp to train a classifier that is approximately invariant to local perturbations along the manifold. The idea of manifold learning using graph-based methods has most recently been combined with kernel (SVM) methods in the Atlas RBF model \citep{pitelis2014} and provides amongst most competitive performance currently available.

In this paper, we instead, choose to exploit the power of \textit{generative models}, which recognise the semi-supervised learning problem as a specialised missing data imputation task for the classification problem.
Existing generative approaches based on models such as Gaussian mixture or hidden Markov models \citep{zhu2006semitut}, have not been very successful due to the need for a large number of mixtures components or states to perform well. More recent solutions have used non-parametric density models, either based on trees \citep{kemp2003semi} or Gaussian processes \citep{adams2009archipelago}, but scalability and accurate inference for these approaches is still lacking. Variational approximations for semi-supervised clustering have also been explored previously \citep{wang2009rate, li2009variational}.

Thus, while a small set of generative approaches have been previously explored, a generalised and scalable probabilistic approach for semi-supervised learning is still lacking. It is this gap that we address through the following contributions:
\begin{itemize}
	\vspace{-2mm}
	\setlength{\itemsep}{1pt}\setlength{\parskip}{0pt} \setlength{\parsep}{0pt}
	\item We describe a new framework for semi-supervised learning with generative models, employing rich parametric density estimators formed by the fusion of probabilistic modelling and deep neural networks.
	\item We show for the first time how variational inference can be brought to bear upon the problem of semi-supervised classification. In particular, we develop a stochastic variational inference algorithm that allows for joint optimisation of both model and variational parameters, and that is scalable to large datasets.
	\item We demonstrate the performance of our approach on a number of data sets providing state-of-the-art results on benchmark problems.
	\item We show qualitatively generative semi-supervised models learn to separate the data classes (content types) from the intra-class variabilities (styles), allowing in a very straightforward fashion to simulate analogies of images on a variety of datasets.
\end{itemize}


==> nips2014-semisupervised copy/macros.tex <==
% Package setup and macros

\usepackage[sort&compress, round, authoryear]{natbib}
\usepackage{amsmath, amsthm}
\usepackage{amsfonts}
\usepackage{amssymb}

\usepackage[pdftex]{graphicx} % more modern
%\usepackage{subfigure} 
\usepackage{subcaption}
\graphicspath{{figures/}} 

%\usepackage{algpseudocode}
\usepackage{algorithm} 
\usepackage{algorithmic}
\usepackage{hyperref}
\usepackage{balance}
\usepackage{url}
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Package for highlighting text
\usepackage{soul}


% Generic math notations
\newcommand{\assign}{:=}
\newcommand{\eqsp}{\,}	% equal space between equations and punctuation
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\proc}[1]{\textsc{#1}}
\newcommand{\categorical}{\text{Cat}}

\newcommand{\E}{\mathbb{E}} %expectation
\newcommand{\FE}{\mathcal{F}} %free energy
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\Tr}{Tr} %matrix trace
\DeclareMathOperator{\diag}{diag} %matrix trace

\let\oldthebibliography=\thebibliography
  \let\endoldthebibliography=\endthebibliography
  \renewenvironment{thebibliography}[1]{%
    \begin{oldthebibliography}{#1}%
      \setlength{\parskip}{0.5ex}%
      \setlength{\itemsep}{0ex}%
}{\end{oldthebibliography}}


\newcommand{\N}{\mathcal{N}} % Gaussian
\newcommand{\D}{\mathcal{D}} % data set


%\usepackage[usenames]{color}
\definecolor{darkblue}{rgb}{0,0.05,0.35}
\definecolor{darkgreen}{rgb}{0,0.6,0}
\newcommand{\comment}[1]{\textcolor{red}{[#1]}}
\newcommand{\scom}[1]{\textcolor{darkgreen}{[#1]}}
\newcommand{\dcom}[1]{\textcolor{blue}{[#1]}}

% Prob expressions
\newcommand{\Expon}[1]{\mathrm{Expon}\left( #1 \right )}
\newcommand{\Conj}[1]{\mathrm{Conj}\left(#1 s\right)}
\newcommand{\expect}[2]{\mathbb{E}_{#1}\left[#2\right]}

% vector symbols
\newcommand{\myvec}[1]{\mbox{$\mathbf{#1}$}}
\newcommand{\myvecsym}[1]{\mbox{$\boldsymbol{#1}$}}

\newcommand{\vzero}{\mbox{$\myvecsym{0}$}}
\newcommand{\vone}{\mbox{$\myvecsym{1}$}}

\newcommand{\valpha}{\mbox{$\myvecsym{\alpha}$}}
\newcommand{\vbeta}{\mbox{$\myvecsym{\beta}$}}
\newcommand{\vchi}{\mbox{$\myvecsym{\chi}$}}
\newcommand{\vdelta}{\mbox{$\myvecsym{\delta}$}}
\newcommand{\vDelta}{\mbox{$\myvecsym{\Delta}$}}
\newcommand{\vepsilon}{\mbox{$\myvecsym{\epsilon}$}}
\newcommand{\veta}{\mbox{$\myvecsym{\eta}$}}
\newcommand{\vgamma}{\mbox{$\myvecsym{\gamma}$}}
\newcommand{\vGamma}{\mbox{$\myvecsym{\Gamma}$}}
\newcommand{\vmu}{\mbox{$\myvecsym{\mu}$}}
\newcommand{\vlambda}{\mbox{$\myvecsym{\lambda}$}}
\newcommand{\vLambda}{\mbox{$\myvecsym{\Lambda}$}}
\newcommand{\vLambdaBar}{\mbox{$\overline{\vLambda}$}}
\newcommand{\vphi}{\mbox{$\myvecsym{\phi}$}}
\newcommand{\vPhi}{\mbox{$\myvecsym{\Phi}$}}
\newcommand{\vpi}{\mbox{$\boldsymbol{\pi}$}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\mbox{$\myvecsym{\Psi}$}}
\newcommand{\vtheta}{\mbox{$\myvecsym{\theta}$}}
\newcommand{\vTheta}{\mbox{$\myvecsym{\Theta}$}}
\newcommand{\vsigma}{\mbox{$\myvecsym{\sigma}$}}
\newcommand{\vSigma}{\mbox{$\myvecsym{\Sigma}$}}
\newcommand{\vOmega}{\mbox{$\myvecsym{\Omega}$}}
\newcommand{\vtau}{\mbox{$\myvecsym{\tau}$}}

%Indicators of n-th or i-th datapoint
%\newcommand{\vxi}{\mbox{$\myvecsym{\xi}$}}
\newcommand{\vxn}{\vx^{(n)}}
\newcommand{\vzn}{\vz^{(n)}}
\newcommand{\yn}{y^{(n)}}
\newcommand{\vxi}{\vx^{(i)}}
\newcommand{\vzi}{\vz^{(i)}}
\newcommand{\yi}{y^{(i)}}

% The \vx and \vz macro's behave weirdly when used in subscripts. The \bx and \bz below work fine in this case
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\pT}{p_{\theta}}
\newcommand{\pdata}{\widetilde{p}}
\newcommand{\pldata}{\widetilde{p}_l}
\newcommand{\pudata}{\widetilde{p}_u}

\newcommand{\qphi}{q_{\small \mathbf{\phi}}}

\newcommand{\va}{\mbox{$\myvec{a}$}}
\newcommand{\vb}{\mbox{$\myvec{b}$}}
\newcommand{\vc}{\mbox{$\myvec{c}$}}
\newcommand{\vd}{\mbox{$\myvec{d}$}}
\newcommand{\ve}{\mbox{$\myvec{e}$}}
\newcommand{\vf}{\mbox{$\myvec{f}$}}
\newcommand{\vg}{\mbox{$\myvec{g}$}}
\newcommand{\vh}{\mbox{$\myvec{h}$}}
\newcommand{\vj}{\mbox{$\myvec{j}$}}
\newcommand{\vk}{\mbox{$\myvec{k}$}}
\newcommand{\vm}{\mbox{$\myvec{m}$}}
\newcommand{\vn}{\mbox{$\myvec{n}$}}
\newcommand{\vp}{\mbox{$\myvec{p}$}}
\newcommand{\vq}{\mbox{$\myvec{q}$}}
\newcommand{\vr}{\mbox{$\myvec{r}$}}
\newcommand{\vs}{\mbox{$\myvec{s}$}}
\newcommand{\vt}{\mbox{$\myvec{t}$}}
\newcommand{\vu}{\mbox{$\myvec{u}$}}
\newcommand{\vv}{\mbox{$\myvec{v}$}}
\newcommand{\vw}{\mbox{$\myvec{w}$}}
\newcommand{\vws}{\mbox{$\vw_s$}}
\newcommand{\vwh}{\mbox{$\hat{\vw}$}}
\newcommand{\vx}{\mbox{$\myvec{x}$}}
\newcommand{\vxt}{\mbox{$\myvec{\tilde{x}}$}}
\newcommand{\vy}{\mbox{$\myvec{y}$}}
\newcommand{\vyt}{\mbox{$\myvec{\tilde{y}}$}}
\newcommand{\vz}{\mbox{$\myvec{z}$}}

\newcommand{\vA}{\mbox{$\myvec{A}$}}
\newcommand{\vB}{\mbox{$\myvec{B}$}}
\newcommand{\vC}{\mbox{$\myvec{C}$}}
\newcommand{\vD}{\mbox{$\myvec{D}$}}
\newcommand{\vE}{\mbox{$\myvec{E}$}}
\newcommand{\vF}{\mbox{$\myvec{F}$}}
\newcommand{\vG}{\mbox{$\myvec{G}$}}
\newcommand{\vH}{\mbox{$\myvec{H}$}}
\newcommand{\vI}{\mbox{$\myvec{I}$}}
\newcommand{\vJ}{\mbox{$\myvec{J}$}}
\newcommand{\vK}{\mbox{$\myvec{K}$}}
\newcommand{\vL}{\mbox{$\myvec{L}$}}
\newcommand{\vM}{\mbox{$\myvec{M}$}}
\newcommand{\vN}{\mbox{$\myvec{N}$}}
\newcommand{\vO}{\mbox{$\myvec{O}$}}
\newcommand{\vP}{\mbox{$\myvec{P}$}}
\newcommand{\vQ}{\mbox{$\myvec{Q}$}}
\newcommand{\vR}{\mbox{$\myvec{R}$}}
\newcommand{\vS}{\mbox{$\myvec{S}$}}
\newcommand{\vT}{\mbox{$\myvec{T}$}}
\newcommand{\vU}{\mbox{$\myvec{U}$}}
\newcommand{\vV}{\mbox{$\myvec{V}$}}
\newcommand{\vW}{\mbox{$\myvec{W}$}}
\newcommand{\vX}{\mbox{$\myvec{X}$}}
%\newcommand{\vXs}{\mbox{$\vX_{\vs}$}}
\newcommand{\vXs}{\mbox{$\vX_{s}$}}
\newcommand{\vXt}{\mbox{$\myvec{\tilde{X}}$}}
\newcommand{\vY}{\mbox{$\myvec{Y}$}}
\newcommand{\vZ}{\mbox{$\myvec{Z}$}}

%Latex theorem/proposition/lemma environments
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

% Specific free energy macro's
\newcommand{\Fl}{\mathcal{L}}
\newcommand{\Fu}{\mathcal{U}}
%\newcommand{\Fl}{\mathcal{F}_{labeled}}
%\newcommand{\Fu}{\mathcal{F}_{unlabeled}}


\makeatletter
\def\blfootnote{\xdef\@thefnmark{}\@footnotetext}
\makeatother


==> nips2014-semisupervised copy/model.tex <==
\section{Deep Generative Models for Semi-supervised Learning}\label{sec:models}
\vspace{-2mm}
We are faced with data that appear as pairs $(\vX, \vY) = \{ (\vx_1, y_1), \ldots, (\vx_N, y_N)\}$, with the $i$-th observation $\vx_i \in \mathbb{R}^D$ and the corresponding class label $y_i \in \{1, \ldots, L\}$. 
Observations will have corresponding latent variables, which we denote by $\vz_i$.
We will omit the index $i$ whenever it is clear that we are referring to terms associated with a single data point. In semi-supervised classification, only a subset of the observations have corresponding class labels; we refer to the empirical distribution over the labelled and unlabelled subsets as $\pldata(\bx,y)$ and $\pudata(\bx)$, respectively. 
We now develop models for semi-supervised learning that exploit generative descriptions of the data to improve upon the classification performance that would be obtained using the labelled data alone.

\textbf{Latent-feature discriminative model (M1):}
A commonly used approach is to construct a model that provides an embedding or feature representation of the data. Using these features, a separate classifier is thereafter trained. The embeddings allow for a clustering of related observations in a latent feature space that allows for accurate classification, even with a limited number of labels. Instead of a linear embedding, or features obtained from a regular auto-encoder, we construct a deep generative model of the data that is able to provide a more robust set of latent features.
The generative model we use is:
\begin{eqnarray}
&p(\vz) =  \N(\vz | \vzero, \vI); \qquad \pT(\vx|\vz) =  f(\vx; \vz, \vtheta),
\label{eq:discriminativeModel}
\end{eqnarray}
where $f(\vx; \vz, \vtheta)$ is a suitable likelihood function (e.g., a Gaussian or Bernoulli distribution) whose probabilities are formed by a non-linear transformation, with parameters $\vtheta$, of a set of latent variables $\vz$. This non-linear transformation is essential to allow for higher moments of the data to be captured by the density model, and we choose these non-linear functions to be deep neural networks.
Approximate samples from the posterior distribution over the latent variables $p(\vz | \vx)$ are used as features to train a classifier that predicts class labels $y$, such as a (transductive) SVM or multinomial regression. 
Using this approach, we can now perform classification in a lower dimensional space since we typically use latent variables whose dimensionality is much less than that of the observations. These low dimensional embeddings should now also be more easily separable since we make use of independent latent Gaussian posteriors whose parameters are formed by a sequence of non-linear transformations of the data. This simple approach results in improved performance for SVMs, and we demonstrate this in section \ref{sect:results}.

\textbf{Generative semi-supervised model (M2):} We propose a probabilistic model that describes the data as being generated by a latent class variable $y$ in addition to a continuous latent variable $\vz$. The data is explained by the generative process:
\begin{align}
p(y) = \textrm{Cat}(y| \vpi);\qquad
p(\vz) = \N(\vz | \vzero, \vI);\qquad
\pT(\vx|y,\vz) = f(\vx; y, \vz, \vtheta), \label{eq:condGenerativeModel}
\end{align}
where $\textrm{Cat}(y | \vpi )$ is the multinomial distribution, the class labels $y$ are treated as latent variables if no class label is available and $\vz$ are additional latent variables. 
These latent variables are marginally independent and allow us, in case of digit generation for example, to separate the class specification from the writing style of the digit.
As before, $f(\vx; y, \vz, \vtheta)$ is a suitable likelihood function, e.g., a Bernoulli or Gaussian distribution, parameterised by a non-linear transformation of the latent variables. In our experiments, we choose deep neural networks as this non-linear function. Since most labels $y$ are unobserved, we integrate over the class of any unlabelled data during the inference process, thus performing classification as inference. Predictions for any missing labels are obtained from the inferred posterior distribution $\pT(y | \vx)$. This model can also be seen as a hybrid continuous-discrete mixture model where the different mixture components share parameters.

\textbf{Stacked generative semi-supervised model (M1+M2):} We can combine these two approaches by first learning a new latent representation $\vz_1$ using the generative model from M1, and subsequently learning a generative semi-supervised model M2, using embeddings from $\vz_1$ instead of the raw data $\vx$. The result is a deep generative model with two layers of stochastic variables: $\pT(\vx,y,\vz_1,\vz_2) = p(y)p(\vz_2)\pT(\vz_1|y,\vz_2)\pT(\vx|\vz_1)$, where the priors $p(y)$ and $p(\vz_2)$ equal those of $y$ and $\vz$ above, and both $\pT(\vz_1|y,\vz_2)$ and $\pT(\vx|\vz_1)$ are parameterised as deep neural networks.


==> nips2014-semisupervised copy/relatedWork.tex <==
\section{Related Work}

We outlined the broad set of existing approaches in the introduction, and describe further some of the approaches that form the state of the art.
In \citet{larochelle2008classification}, Discriminative Restricted Boltzmann Machines model the joint distribution of an input vector and the target class.
In \citet{weston2012deep}, the weights of all layers are trained by minimizing the combined loss function of a global supervised task and a semi-supervised embedding as a regularizer.

Some semi-supervised methods make use of ‘cluster assumption’, i.e. that the decision boundary should lie in low-density regions \citet{chapelle2004semi}.
Deep semi-supervised Embedding \citep{weston2012deep} learns a deep classifier, which is regularised with all (labelled and unlabelled) datapoints by encouraging similar datapoints (with same class label) to have similar hidden-unit activations, while pulling away from some random unlabeled datapoint. 

The Manifold Tangent Classifier (MTC) \citep{rifai2011manifold} trains contrastive auto-encoders to learn the manifold on which the data lies. It then uses Tangent Prop to train a classifier that is approximately invariant to local perturbations along the manifold.
In \citet{lee2013}, the authors employ Pseudo-Label (PL), a rediscovery of Entropy Regularization \citep{grandvalet2006} for semi-supervised learning. By minimizing the conditional entropy of the class labels for the unlabelled data points, the method favours a low-density separation between classes, a commonly assumed prior for semi-supervised learning \citep{chapelle2004semi}.  The Pseudo-Label method is combined with dropout and Denoising AE to boost performance. However, the experimental results are invalid since hyper-parameters were tuned on a (large) validation set.

==> nips2014-semisupervised copy/results.tex <==
\vspace{-2mm}
\section{Experimental Results}
\label{sect:results}
Open source code, with which the most important results and figures can be reproduced, is available at \url{http://github.com/dpkingma/nips14-ssl}. For the latest experimental results, please see \url{http://arxiv.org/abs/1406.5298}.
%
\vspace{-2mm}
\subsection{Benchmark Classification}
\vspace{-2mm}
We test performance on the standard MNIST digit classification benchmark. The data set for semi-supervised learning is created by splitting the 50,000 training points between a labelled and unlabelled set, and varying the size of the labelled  from 100 to 3000. We ensure that all classes are balanced when doing this, i.e. each class has the same number of labelled points. We create a number of data sets using randomised sampling to confidence bounds for the mean performance under repeated draws of data sets.
%In this benchmark, each model is trained on the training set of 50,000 images and randomly sampled subset of labels, where we made sure that an even number of labels were sampled per class. So in case of 100 labels and 10 classes, there were 10 labels per class.

For model M1 we used a 50-dimensional latent variable $\vz$. The MLPs that form part of the generative and inference models were constructed with two hidden layers, each with 600 hidden units, using softplus $\log (1+e^x)$ activation functions. On top, a transductive SVM (TSVM) was learned on values of $\vz$ inferred with $\qphi(\vz|\vx)$. For model M2 we also used 50-dimensional $\vz$.  In each experiment, the MLPs were constructed with one hidden layer, each with 500 hidden units and softplus activation functions. In case of SVHN and NORB, we found it helpful to pre-process the data with PCA. This makes the model one level deeper, and still optimizes a lower bound on the likelihood of the unprocessed data.

Table \ref{tab:mnistComparison} shows classification results. We compare to a broad range of existing solutions in semi-supervised learning, in particular to classification using nearest neighbours (NN), support vector machines on the labelled set (SVM), the transductive SVM (TSVM), and contractive auto-encoders (CAE). Some of the best results currently are obtained by the manifold tangent classifier (MTC) \citep{rifai2011manifold} and the AtlasRBF method~\citep{pitelis2014}. %Results in the table for these methods are reproduced from \citet{rifai2011manifold}.
Unlike the other models in this comparison, our models are fully probabilistic but have a cost in the same order as these alternatives.
%We also provide confidence bounds to the mean performance under repeated draws of data sets.

\paragraph{Results:} The latent-feature discriminative model (M1) performs better than other models based on simple embeddings of the data, demonstrating the effectiveness of the latent space in providing robust features that allow for easier classification. By combining these features with a classification mechanism directly in the same model, as in the conditional generative model (M2), we are able to get similar results without a separate TSVM classifier.

However, by far the best results were obtained using the stack of models M1 and M2. This combined model provides accurate test-set predictions across all conditions, and easily outperforms the previously best methods. 
We also tested this deep generative model for supervised learning with all available labels, and obtain a test-set performance of 0.96\%, which is among the best published results for this permutation-invariant MNIST classification task.

%providing new state-of-the-art result for semi-supervised classification on this data set.
%\comment{Since results on MTC, the closest competitor, were based on a single noisy sample [source: private communication] as opposed to our numbers that are based on a much more rigorous sample, our method can be regarded as state-of-the-art for semi-supervised classification on this data set.}

%\comment{Experiments with 3000 labels will be included in this the final paper, but were not finished yet at time of submission.}

\begin{table}[tp]
	\centering
	\caption{Benchmark results of semi-supervised classification on MNIST with few labels.}
	\scriptsize
	\begin{tabular}{l|llllll |lll}
		\hline
		$N$ & NN & CNN  & TSVM &  CAE & MTC & AtlasRBF & M1+TSVM & M2 & M1+M2\\
		\hline \hline
		100 & 25.81 & 22.98 & 16.81  & 13.47 & 12.03 & 8.10 ($\pm$ 0.95)  & 11.82 ($\pm$ 0.25) & 11.97 ($\pm$ 1.71) & \textbf{3.33} ($\pm$ 0.14) \\
		600 & 11.44 & 7.68 & 6.16  & 6.3 & 5.13   &  -- &  5.72 ($\pm$ 0.049) & 4.94 ($\pm$ 0.13) & \textbf{2.59} ($\pm$ 0.05) \\
		1000 & 10.7 & 6.45 & 5.38  & 4.77 & 3.64  & 3.68 ($\pm$ 0.12)  &  4.24 ($\pm$ 0.07) & 3.60 ($\pm$ 0.56) & \textbf{2.40} ($\pm$ 0.02) \\
	 	3000 & 6.04 & 3.35 & 3.45  & 3.22 & 2.57 &  -- &  3.49 ($\pm$ 0.04) & 3.92 ($\pm$ 0.63) & \textbf{2.18} ($\pm$ 0.04) \\
		\hline
	\end{tabular}
	\label{tab:mnistComparison}
	\vspace{-5mm}
\end{table}


\subsection{Conditional Generation}
\vspace{-2mm}
The conditional generative model can be used to explore the underlying structure of the data, which we demonstrate through two forms of analogical reasoning.
Firstly, we demonstrate style and content separation by fixing the class label $y$, and then varying the latent variables $\vz$ over a range of values. Figure \ref{fig:analogies} shows three MNIST classes in which, using a trained model with two latent variables, and the 2D latent variable varied over a range from -5 to 5. In all cases, we see that nearby regions of latent space correspond to similar writing styles, independent of the class; the left region represents upright writing styles, while the right-side represents slanted styles.
%We also show a similar visualisation for the street view house numbers (SVHN) data set \citep{SVHNdata}, which consists of more than 70,000 images of house numbers, in figure \ref{fig:analogies} (top). Here we use a 300-dimensional latent variable; each column represents a class label, and we show a number of independent samples generated from the model in each row. We show similar results for the NORB image recognition data set in figure \ref{fig:analogies}(top), where again each column represents one of the five main classes. These results show that our model has learned to capture the global luminance and rotation of the images in a purely unsupervised way. This opens up interesting possibilities for pose estimation using generative models.

%\begin{figure}[t]
%\centering
%\begin{minipage}{1.0 \textwidth}
%\begin{figure}[H]
%\centering
%\includegraphics[height =4cm]{handwriting2_bw}
%\hspace{2mm}
%\includegraphics[height =4cm]{handwriting3_bw}
%\hspace{2mm}
%\includegraphics[height =4cm]{handwriting4_bw}
%%\hspace{2mm}
%%\includegraphics[height =2cm]{handwriting5_bw}
%\caption{Handwriting styles for MNIST obtained by fixing the class label and varying the latent variable over a 2D grid. 
%}
%\label{fig:mnsitGeneration}
%\end{figure}
%\end{minipage}
%\vspace{-5mm}
%\end{figure}
%

As a second approach, we use a test image and pass it through the inference network to infer a value of the latent variables corresponding to that image. We then fix the latent variables $\vz$ to this value, vary the class label $\vy$, and simulate images from the generative model corresponding to that combination of $\vz$ and $\vy$. This again demonstrate the disentanglement of style from class. Figure~\ref{fig:analogies} shows these analogical fantasies for the MNIST and SVHN datasets \citep{netzer2011reading}. The SVHN data set is a far more complex data set than MNIST, but the model is able to fix the style of house number and vary the digit that appears in that style well. These generations represent the best current performance in simulation from generative models on these data sets.

The model used in this way also provides an alternative model to the stochastic feed-forward networks (SFNN) described by \citet{tang2013learning}. The performance of our model significantly improves on SFNN, since instead of an inefficient Monte Carlo EM algorithm relying on importance sampling, we are able to perform efficient joint inference that is easy to scale.

%\begin{figure}[t]
%\begin{minipage}{.6\textwidth}
%  %\centering
%  \begin{figure}[H]
%  \centering
%  \includegraphics[width = 6cm]{svhn_crop_p3}\\
%  \vspace{2mm}
%  \includegraphics[width = 6cm]{svhn_crop_p1}\\
%  \includegraphics[width = 6cm]{svhn_crop_p2}
%  \caption{Analogical reasoning on SVHN. (Top) Fixed class per col., (Bottom) Fixed latent var. (style) per row.}
%  \label{fig:svhnAnalogies}
%  \end{figure}
%  \end{minipage}%
%  \hskip3ex
%  %\vskip-0ex
%  \begin{minipage}{.3\textwidth}
%  %\centering
%  \begin{figure}[H]
%  \centering
%   \includegraphics[width = 3.1cm]{norb_crop}\\
%   \vspace{2mm}
%  	\includegraphics[width = 3.1cm]{norb_analogy_crop}
%  	\caption{Analogical reasoning for NORB.}
%   	\label{fig:norbAnalogies}
%  \end{figure}
%\end{minipage}%
%\vspace{-3mm}
%\end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.99\textwidth}\centering
\includegraphics[width=12.4cm]{handwriting_together}
\caption{Handwriting styles for MNIST obtained by fixing the class label and varying the 2D latent variable $\vz$}
\end{subfigure}
\vspace{2.5mm}\\
\begin{subfigure}[t]{0.49\textwidth}\centering
\includegraphics[width=6.2cm]{analogies_mnist/together}
\caption{MNIST analogies}
\end{subfigure}
\begin{subfigure}[t]{0.49\textwidth}\centering
\includegraphics[width=6.2cm]{analogies_svhn/together}
\caption{SVHN analogies}
\end{subfigure}
\caption{\textbf{(a)} Visualisation of handwriting styles learned by the model with 2D $\vz$-space. \textbf{(b,c)} Analogical reasoning with generative semi-supervised models using a high-dimensional $\vz$-space. The leftmost columns show images from the test set. The other columns show analogical fantasies of $\vx$ by the generative model, where the latent variable $\vz$ of each row is set to the value inferred from the test-set image on the left by the inference network. Each column corresponds to a class label $\vy$.}
\label{fig:analogies}
\end{figure}

%
\subsection{Image Classification}
\vspace{-2mm}
We demonstrate the performance of image classification on the SVHN, and  NORB image data sets. Since no comparative results in the semi-supervised setting exists, we perform nearest-neighbour and TSVM classification with RBF kernels and compare performance on features generated by our latent-feature discriminative model to the original features. The results are presented in tables~\ref{tab:svhn} and~\ref{tab:norb}, and we again demonstrate the effectiveness of our approach for semi-supervised classification.

\begin{table}
\parbox{.45\linewidth}{
	\centering
	\caption{Semi-supervised classification on the SVHN dataset with 1000 labels.}
\scriptsize
	\begin{tabular}{cc|cccc}
		\hline
		KNN & TSVM & M1+KNN  & M1+TSVM & M1+M2\\
		\hline \hline
		77.93 & 66.55 & 65.63 & 54.33 & \textbf{36.02} \\
		($\pm$ 0.08) & ($\pm$ 0.10) & ($\pm$ 0.15) & ($\pm$ 0.11) & ($\pm$ 0.10)
	\end{tabular}
	\label{tab:svhn}
}
\hfill
\parbox{.45\linewidth}{
	\centering
	\caption{Semi-supervised classification on the NORB dataset with 1000 labels.}
\scriptsize
	\begin{tabular}{cc|cccc}
		\hline
		KNN & TSVM & M1+KNN & M1+TSVM  \\
		\hline \hline
		78.71  & 26.00  & 65.39  & \textbf{18.79}  \\
		($\pm$ 0.02) & ($\pm$ 0.06) & ($\pm$ 0.09) & ($\pm$ 0.05)
	\end{tabular}
	\label{tab:norb}
}
	
	
	\vspace{-5mm}
\end{table}

\subsection{Optimization details} The parameters were initialized by sampling randomly from $\N(\vzero,0.001^2\vI)$, except for the bias parameters which were initialized as 0. The objectives were optimized using minibatch gradient ascent until convergence, using a variant of RMSProp with momentum and initialization bias correction, a constant learning rate of $0.0003$, first moment decay (momentum) of $0.1$, and second moment decay of $0.001$. For MNIST experiments, minibatches for training were generated by treating normalised pixel intensities of the images as Bernoulli probabilities and sampling binary images from this distribution.
In the M2 model, a weight decay was used corresponding to a prior of $(\vtheta, \vphi) \sim \mathcal{N}(0,I)$. 



==> relatedWork.tex <==
\section{Related Work}

We outlined the broad set of existing approaches in the introduction, and describe further some of the approaches that form the state of the art.
In \citet{larochelle2008classification}, Discriminative Restricted Boltzmann Machines model the joint distribution of an input vector and the target class.
In \citet{weston2012deep}, the weights of all layers are trained by minimizing the combined loss function of a global supervised task and a semi-supervised embedding as a regularizer.

Some semi-supervised methods make use of ‘cluster assumption’, i.e. that the decision boundary should lie in low-density regions \citet{chapelle2004semi}.
Deep semi-supervised Embedding \citep{weston2012deep} learns a deep classifier, which is regularised with all (labelled and unlabelled) datapoints by encouraging similar datapoints (with same class label) to have similar hidden-unit activations, while pulling away from some random unlabeled datapoint. 

The Manifold Tangent Classifier (MTC) \citep{rifai2011manifold} trains contrastive auto-encoders to learn the manifold on which the data lies. It then uses Tangent Prop to train a classifier that is approximately invariant to local perturbations along the manifold.
In \citet{lee2013}, the authors employ Pseudo-Label (PL), a rediscovery of Entropy Regularization \citep{grandvalet2006} for semi-supervised learning. By minimizing the conditional entropy of the class labels for the unlabelled data points, the method favours a low-density separation between classes, a commonly assumed prior for semi-supervised learning \citep{chapelle2004semi}.  The Pseudo-Label method is combined with dropout and Denoising AE to boost performance. However, the experimental results are invalid since hyper-parameters were tuned on a (large) validation set.
